Fast Spectral Ranking for Similarity Search

Despite the success of deep learning on representing images for particular object retrieval, recent studies show that the learned representations still lie on manifolds in a high dimensional space. This makes the Euclidean nearest neighbor search biased for this task. Exploring the manifolds online remains expensive even if a nearest neighbor graph has been computed offline. This work introduces an explicit embedding reducing manifold search to Euclidean search followed by dot product similarity search. This is equivalent to linear graph filtering of a sparse signal in the frequency domain. To speed up online search, we compute an approximate Fourier basis of the graph offline. We improve the state of art on particular object retrieval datasets including the challenging Instre dataset containing small objects. At a scale of 10^5 images, the offline cost is only a few hours, while query time is comparable to standard similarity search.

==> figs/low-pass/tex/abbrev.tex <==
% symbol abbreviations

\newcommand{\figfile}[1]{fig/#1}
\newcommand{\eval}[1]{\the\numexpr#1\relax}
\newcommand{\head}[1]{{\smallskip\noindent\bf #1}}

\newcommand<>{\white}  [2][100]{{\color#3  {white!#1}{#2}}}
\newcommand<>{\red}    [2][100]{{\color#3    {red!#1}{#2}}}
\newcommand<>{\blue}   [2][100]{{\color#3   {blue!#1}{#2}}}
\newcommand<>{\green}  [2][100]{{\color#3  {green!#1}{#2}}}
\newcommand<>{\cyan}   [2][100]{{\color#3   {cyan!#1}{#2}}}
\newcommand<>{\yellow} [2][100]{{\color#3 {yellow!#1}{#2}}}
\newcommand<>{\magenta}[2][100]{{\color#3{magenta!#1}{#2}}}
\newcommand<>{\orange} [2][100]{{\color#3 {orange!#1}{#2}}}
\newcommand<>{\gray}   [2][100]{{\color#3   {gray!#1}{#2}}}

\newcommand<>{\dwhite}  [2][100]{{\color#3  {white!#1!black}{#2}}}
\newcommand<>{\dred}    [2][100]{{\color#3    {red!#1!black}{#2}}}
\newcommand<>{\dblue}   [2][100]{{\color#3   {blue!#1!black}{#2}}}
\newcommand<>{\dgreen}  [2][100]{{\color#3  {green!#1!black}{#2}}}
\newcommand<>{\dcyan}   [2][100]{{\color#3   {cyan!#1!black}{#2}}}
\newcommand<>{\dyellow} [2][100]{{\color#3 {yellow!#1!black}{#2}}}
\newcommand<>{\dmagenta}[2][100]{{\color#3{magenta!#1!black}{#2}}}
\newcommand<>{\dorange} [2][100]{{\color#3 {orange!#1!black}{#2}}}
\newcommand<>{\dgray}   [2][100]{{\color#3   {gray!#1!black}{#2}}}

\newcommand{\tta}[1]{\texttt{\alert{#1}}}
\newcommand{\qu}[1]{\textrm{\textbf{\Large{\alert{#1}}}}}
\newcommand{\quot}[1]{\qu{``}\texttt{#1}\qu{''}}
\newcommand{\inde}[1]{\begin{itemize}\item[]{#1}\end{itemize}}

\newcommand{\refc}[1]{\gray{#1}}
\newcommand{\tb}[1]{{\textbf{#1}}}
\newcommand{\equ}[1]{(\ref{equ:#1})\xspace}

\newenvironment{colsep}[1]{\setlength{\tabcolsep}{#1}}{\setlength{\tabcolsep}{6pt}}

%--------------------------------------------------------------------

\newcommand{\tran}{^\top}
\newcommand{\mtran}{^{-\top}}
\newcommand{\zcol}{\mathbf{0}}
\newcommand{\zrow}{\zcol\tran}

\newcommand{\ind}{\mathbbm{1}}
\newcommand{\expect}{\mathbb{E}}
\newcommand{\nat}{\mathbb{N}}
\newcommand{\zahl}{\mathbb{Z}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\proj}{\mathbb{P}}
\newcommand{\prob}{\mathbf{Pr}}

\newcommand{\mif}{\textrm{if }}
\newcommand{\minimize}{\textrm{minimize }}
\newcommand{\maximize}{\textrm{maximize }}
\newcommand{\st}{\textrm{subject to }}

\newcommand{\id}{\operatorname{id}}
\newcommand{\const}{\operatorname{const}}
\newcommand{\sgn}{\operatorname{sgn}}
\newcommand{\var}{\operatorname{Var}}
\newcommand{\mean}{\operatorname{mean}}
\newcommand{\trace}{\operatorname{tr}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\vect}{\operatorname{vec}}
\newcommand{\cov}{\operatorname{cov}}

\newcommand{\defn}{\mathrel{:=}}
\newcommand{\peq}{\mathrel{+\!=}}
\newcommand{\meq}{\mathrel{-\!=}}

\newcommand{\floor}[1]{\left\lfloor{#1}\right\rfloor}
\newcommand{\ceil}[1]{\left\lceil{#1}\right\rceil}
\newcommand{\inner}[1]{\left\langle{#1}\right\rangle}
\newcommand{\norm}[1]{\left\|{#1}\right\|}
\newcommand{\frob}[1]{\norm{#1}_F}
\newcommand{\card}[1]{\left|{#1}\right|\xspace}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\der}[3][]{\frac{d^{#1}#2}{d#3^{#1}}}
\newcommand{\pder}[3][]{\frac{\partial^{#1}{#2}}{\partial{#3^{#1}}}}
\newcommand{\dder}[3]{\frac{\partial^2{#1}}{\partial{#2}\partial{#3}}}

\newcommand{\wb}[1]{\overline{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}

\def\spsx{\hspace{1pt}}
\def\sps{\hspace{2pt}}
\def\spm{\hspace{5pt}}
\def\spl{\hspace{10pt}}
\def\splx{\hspace{20pt}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\va}{\mathbf{a}}
\newcommand{\vb}{\mathbf{b}}
\newcommand{\vc}{\mathbf{c}}
\newcommand{\vd}{\mathbf{d}}
\newcommand{\ve}{\mathbf{e}}
\newcommand{\vf}{\mathbf{f}}
\newcommand{\vg}{\mathbf{g}}
\newcommand{\vh}{\mathbf{h}}
\newcommand{\vi}{\mathbf{i}}
\newcommand{\vj}{\mathbf{j}}
\newcommand{\vk}{\mathbf{k}}
\newcommand{\vl}{\mathbf{l}}
\newcommand{\vm}{\mathbf{m}}
\newcommand{\vn}{\mathbf{n}}
\newcommand{\vo}{\mathbf{o}}
\newcommand{\vp}{\mathbf{p}}
\newcommand{\vq}{\mathbf{q}}
\newcommand{\vr}{\mathbf{r}}
\newcommand{\vs}{\mathbf{s}}
\newcommand{\vt}{\mathbf{t}}
\newcommand{\vu}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vw}{\mathbf{w}}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\vz}{\mathbf{z}}

\newcommand{\vA}{\mathbf{A}}
\newcommand{\vB}{\mathbf{B}}
\newcommand{\vC}{\mathbf{C}}
\newcommand{\vD}{\mathbf{D}}
\newcommand{\vE}{\mathbf{E}}
\newcommand{\vF}{\mathbf{F}}
\newcommand{\vG}{\mathbf{G}}
\newcommand{\vH}{\mathbf{H}}
\newcommand{\vI}{\mathbf{I}}
\newcommand{\vJ}{\mathbf{J}}
\newcommand{\vK}{\mathbf{K}}
\newcommand{\vL}{\mathbf{L}}
\newcommand{\vM}{\mathbf{M}}
\newcommand{\vN}{\mathbf{N}}
\newcommand{\vO}{\mathbf{O}}
\newcommand{\vP}{\mathbf{P}}
\newcommand{\vQ}{\mathbf{Q}}
\newcommand{\vR}{\mathbf{R}}
\newcommand{\vS}{\mathbf{S}}
\newcommand{\vT}{\mathbf{T}}
\newcommand{\vU}{\mathbf{U}}
\newcommand{\vV}{\mathbf{V}}
\newcommand{\vW}{\mathbf{W}}
\newcommand{\vX}{\mathbf{X}}
\newcommand{\vY}{\mathbf{Y}}
\newcommand{\vZ}{\mathbf{Z}}

\newcommand{\vone}{\mathbf{1}}
\newcommand{\vzero}{\mathbf{0}}

\newcommand{\valpha}{{\boldsymbol{\alpha}}}
\newcommand{\vbeta}{{\boldsymbol{\beta}}}
\newcommand{\vgamma}{{\boldsymbol{\gamma}}}
\newcommand{\vdelta}{{\boldsymbol{\delta}}}
\newcommand{\vepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\vzeta}{{\boldsymbol{\zeta}}}
\newcommand{\veta}{{\boldsymbol{\eta}}}
\newcommand{\vtheta}{{\boldsymbol{\theta}}}
\newcommand{\viota}{{\boldsymbol{\iota}}}
\newcommand{\vkappa}{{\boldsymbol{\kappa}}}
\newcommand{\vlambda}{{\boldsymbol{\lambda}}}
\newcommand{\vmu}{{\boldsymbol{\mu}}}
\newcommand{\vnu}{{\boldsymbol{\nu}}}
\newcommand{\vxi}{{\boldsymbol{\xi}}}
\newcommand{\vomikron}{{\boldsymbol{\omikron}}}
\newcommand{\vpi}{{\boldsymbol{\pi}}}
\newcommand{\vrho}{{\boldsymbol{\rho}}}
\newcommand{\vsigma}{{\boldsymbol{\sigma}}}
\newcommand{\vtau}{{\boldsymbol{\tau}}}
\newcommand{\vupsilon}{{\boldsymbol{\upsilon}}}
\newcommand{\vphi}{{\boldsymbol{\phi}}}
\newcommand{\vchi}{{\boldsymbol{\chi}}}
\newcommand{\vpsi}{{\boldsymbol{\psi}}}
\newcommand{\vomega}{{\boldsymbol{\omega}}}

\newcommand{\rLambda}{\mathrm{\Lambda}}
\newcommand{\rSigma}{\mathrm{\Sigma}}

%--------------------------------------------------------------------
% big parentesis

\makeatletter
\newcommand{\vast}[1]{\bBigg@{#1}}
\makeatother

%--------------------------------------------------------------------------------
% column width

\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

%--------------------------------------------------------------------------------
% add a period to the end of an abbreviation unless there's one
% already, then \xspace

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace\xspace}
%
\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\Vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother


==> figs/low-pass/tex/beam.tex <==
% macros for beamer

% replaces "<spec>" by "spec"
\newcommand{\clearbrackets}[1]{\expandafter\inside#1}\def\inside<#1>{#1}

% extends an overlay specification to all modes
\newcommand{\extendspec}[1]{#1|handout:#1|article:#1}
\newcommand{\at}[1]{#1|handout:#1|article:#1}

% clears an overlay specification from "<spec>" to "spec" and then extends to all modes
\newcommand{\onspec}[1]{\extendspec{\clearbrackets{#1}}}

% shortcuts for \includegraphics
\newcommand<>{\figure}[2][1]{\includegraphics#3[width=#1\textwidth]{#2}}
\newcommand<>{\figureh}[2][1]{\includegraphics#3[height=#1\textheight]{#2}}

% shortcuts for \includegraphics, where "name" is replaced by "\figfile{name}"
% \figfile is assumed to exist and return a filename pattern for figures, e.g. "figure3-#1.png"
\newcommand<>{\graph}[2][]{\includegraphics#3[#1]{\figfile{#2}}}
\newcommand<>{\fig}[2][1]{\figure#3[#1]{\figfile{#2}}}
\newcommand<>{\figh}[2][1]{\figureh#3[#1]{\figfile{#2}}}
\newcommand<>{\figon}[2][1]{\fig<\onspec{#3}>[#1]{#2}}
\newcommand<>{\fighon}[2][1]{\figh<\onspec{#3}>[#1]{#2}}

\newcommand<>{\vfig}[2][1]{\visible#3{\fig[#1]{#2}}}

% extend overlay specifications of \only, \onslide and \visible
\newcommand<>{\on}{\only<\onspec{#1}>}
\newcommand<>{\ons}{\onslide<\onspec{#1}>}
\newcommand<>{\vis}{\visible<\onspec{#1}>}

% set handout style
\newcommand{\handstyle}{
  \mode<handout>{
    \usepackage{pgfpages}
    \pgfpagesuselayout{2 on 1}[a4paper,border shrink=5mm]
  }
}

% shortcuts for TOC (main, parts, sections, subsections)
\newcommand{\toc}{
	\begin{frame}
		\frametitle{outline}
		\begin{columns}
			\begin{column}{.9\textwidth}
				%\tableofcontents[pausesections]
				\tableofcontents
			\end{column}
		\end{columns}
	\end{frame}
}

\newcommand{\partheading}{outline -- part \Rmnum{\insertpartnumber}}
\newcommand{\tocpart}{\AtBeginPart{
	\frame{\partpage}
	\begin{frame}
		\frametitle{\partheading}
		\tableofcontents[part=\insertpartnumber,pausesections]
	\end{frame}
}}

\newcommand{\tocsecpart}{\tocsec[\partheading]}
\newcommand{\tocsec}[1][outline]{\AtBeginSection[]{
	\begin{frame}<beamer>
		\frametitle{#1}
		\tableofcontents[currentsection,currentsubsection]
	\end{frame}
}}

\newcommand{\tocsubpart}{\tocsub[\partheading]}
\newcommand{\tocsub}[1][outline]{\AtBeginSubsection[]{
	\begin{frame}<beamer>
		\frametitle{#1}
		\tableofcontents[currentsection,currentsubsection]
	\end{frame}
}}

% roman numerals
\makeatletter
\newcommand{\rmnum}[1]{\romannumeral #1}
\newcommand{\Rmnum}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother

% color boxes for biographies
\setbeamercolor{bioupper}{fg=purple!50!blue!60!black,bg=purple!30!blue!40!white}
\setbeamercolor{biolower}{bg=purple!30!blue!20!white}
\newenvironment{bio}[2]{
	\begin{beamerboxesrounded}[upper=bioupper,lower=biolower,width=\textwidth,shadow=true]{\structure{#1}}
		\begin{columns}
		\column{.3\textwidth} {#2}
		\column{.6\textwidth}
}{
		\end{columns}
	\end{beamerboxesrounded}
}

%--------------------------------------------------------------------

% section frame
\newcommand{\fsect}[2]{%
\begin{frame}\begin{center}
{\white{.}#2\white{.}}\\[2em]{\Huge \structure{#1}}
\end{center}\end{frame}
}

% section definition
\newcommand{\tsect}[3]{%
\renewcommand{\figfile}{#1/fig/}
\section{#2}
\fsect{#2}{#3}
\input{#1/#1}
}

% section with image
\newcommand{\isect}[4][.5]{\tsect{#3}{#4}{\figh[#1]{#2}\\[1em]}}

% plain section
\newcommand{\sect}[2]{\tsect{#1}{#2}{}}


==> figs/low-pass/tex/plots-ext.tex <==
\usepackage{tikzextern}
\usepackage{pgffor}
\newcommand{\extfig}[2]{\tikzsetnextfilename{fig/extern/#1}{#2}}
\newcommand{\extdata}[1]{}


==> figs/low-pass/tex/plots.tex <==
\usepackage{tikz}
\usetikzlibrary{arrows,shapes,calc,matrix,fit,backgrounds,positioning,shapes.multipart,graphs,graphs.standard,shadows,mindmap,scopes,intersections}
\usepackage{chapterfolder}   % finds relative paths in nested \input's
% \usepackage{pgffor}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=1.9}

%-----------------------------------------------------------------------------
% tikz styles

\tikzstyle{every picture}+=[
	remember picture,
	every text node part/.style={align=center},
	every matrix/.append style={ampersand replacement=\&},
]
\tikzstyle{tight} = [inner sep=0pt,outer sep=0pt]
\tikzstyle{txt} = [inner sep=1pt,outer sep=0pt,anchor=base]
\tikzstyle{base} = [baseline,every node/.style={tight,anchor=base}]
\tikzstyle{lab} = [draw=none,fill=blue!10,anchor=base,font=\footnotesize]
\tikzstyle{label} = [baseline,every node/.style={lab}]
\tikzstyle{over} = [overlay,every path/.style={->,draw=red,thick},nodes={draw}]
\tikzstyle{semi} = [draw opacity=.5]
\tikzstyle{paper} = [fill=white]
\tikzstyle{help} = [gray]
\tikzstyle{high} = [blue!70]
\tikzstyle{op} = [draw,circle,tight]
\tikzstyle{dot} = [fill,draw,circle,inner sep=1pt,outer sep=0]
\tikzstyle{circ} = [draw,circle,thick,inner sep=1.5pt,outer sep=0]
\tikzstyle{ocirc} = [draw,circle,thick,inner sep=2pt,outer sep=0]
\tikzstyle{node} = [draw,circle,tight,minimum size=16pt,anchor=center]
\tikzstyle{box} = [draw,thick,rectangle,inner sep=6pt]
\tikzstyle{group} = [high,box,opacity=.5]
\tikzstyle{maths} = [matrix of math nodes]
\tikzstyle{rsep} = [row sep={#1,between origins}]
\tikzstyle{csep} = [column sep={#1,between origins}]
\tikzstyle{short} = [shorten >=#1,shorten <=#1]
\tikzstyle{dim1} = [fill opacity=.3,text opacity=1]
\tikzstyle{dim2} = [fill opacity=.5,text opacity=1]
\tikzstyle{dim3} = [fill opacity=.7,text opacity=1]
\tikzstyle{rectc} = [tight,transform shape]
\tikzstyle{rect} = [rectc,anchor=south west]

%--------------------------------------------------------------------
% style overlays

\newcommand<>{\son}[2]{\alt#3{\tikzset{#1/.style={#2}}}{\tikzset{#1/.style={}}}}
\newcommand<>{\sunc}[2]{\alt#3{\tikzset{#1/.style={#2}}}{\tikzset{#1/.style={#2,opacity=.3}}}}
\newcommand<>{\svis}[2]{\alt#3{\tikzset{#1/.style={#2}}}{\tikzset{#1/.style={#2,opacity=0}}}}
\newcommand<>{\salt}[3]{\alt#4{\tikzset{#1/.style={#2}}}{\tikzset{#1/.style={#3}}}}
\newcommand<>{\stemp}[4]{\temporal#5{\tikzset{#1/.style={#2}}}{\tikzset{#1/.style={#3}}}{\tikzset{#1/.style={#4}}}}

%--------------------------------------------------------------------

% layers
\pgfdeclarelayer{bg4}
\pgfdeclarelayer{bg3}
\pgfdeclarelayer{bg2}
\pgfdeclarelayer{bg1}
\pgfdeclarelayer{fg1}
\pgfdeclarelayer{fg2}
\pgfdeclarelayer{fg3}
\pgfdeclarelayer{fg4}
\pgfsetlayers{bg4,bg3,bg2,bg1,main,fg1,fg2,fg3,fg4}

%--------------------------------------------------------------------

% nested equation/text inside tikz picture, to provide a labeled node
\newcommand{\nequ}[3][]{\tikz[base]{\node[#1] (#2) {$\displaystyle {#3}$};}}
\newcommand{\ntext}[3][]{\tikz[base]{\node[#1] (#2) {{#3}};}}

% apply style #1 to given text #2
\newcommand{\style}[2][]{\tikz[base]{\node[#1]{#2};}}

%--------------------------------------------------------------------

% display physical-to-logical unit ratio (how many pt per 1 logical unit)
\makeatletter
\newcommand\displogical{{%
    \pgfmathparse{1000*\pgf@xx}%
    \pgfmathprintnumber{\pgfmathresult}%
}}
\makeatother

% convert physical units to logical (dimensionless)
\newcommand{\logical}[1]{scalar(#1/28.4527)}
\newcommand{\physical}[1]{#1*28.4527pt}

%-----------------------------------------------------------------------------
% tikz-assisted positioning

% position image as character
\newcommand{\tchar}[2]{%
	\tikz{%
		\node[minimum width=#1\textwidth](a){};
		\node[tight,overlay] at(a) {\fig[#1]{#2}};
	}%
}

% lower object #1 by dimension #2 - useful as a workaround to (manually)
% center objects vertically inside overprint
\newcommand{\low}[2][0pt]{\tikz{\node(a){};\node[below=#1 of a]{#2};}}

% shift given tikz paths #2 by #1
\newcommand{\off}[2][(0pt,0pt)]{\tikz{\node[tight](a){};{[shift={#1}]{#2}}}}

% footer - place text #2 styled as #1 at the bottom left corner of slide
\newcommand{\foot}[2][]{%
	\tikz[overlay]{%
		\node[shift={(2ex,2ex)},anchor=south west,tight,#1]
		at (current page.south west)
		{\begin{varwidth}{\textwidth}{#2}\end{varwidth}};
	}%
}

% citation as footer
\newcommand{\refs}[1]{\foot[black!70]{\tiny {#1}\par}}

% cross out a rectangle specified by two nodes at the corners
% e.g. mark two nodes like \ntext{topleft}{...} and \ntext{bottomright}{...},
% then \crossout{topleft}{bottomright}
\newcommand<>{\crossout}[3][]{
\begin{tikzpicture}[overlay]
	\node[fit=(#2)(#3)](box){};
	\draw#4[red,line width=3pt,#1]
		(box.south west)--(box.north east)
		(box.north west)--(box.south east);
\end{tikzpicture}
}

%-----------------------------------------------------------------------------
% pgfplots general options

\newcommand{\plot}[2]{\cffolderinput{#1}{#2}}
\newcommand{\data}[1]{\cfcurrentfolder #1.txt}
\newcommand{\tabread}[2]{\pgfplotstableread{\data{#1}}#2}

\newcommand{\leg}[1]{\addlegendentry{#1}}
\newcommand{\legtext}[1]{\addlegendimage{empty legend} \addlegendentry{#1}}

%-----------------------------------------------------------------------------
% pgfplots styles

\tikzset{every mark/.append style={solid}}
\pgfplotsset{%smooth,
	grid=both, width=\columnwidth, try min ticks=5,
% 	every axis x label/.style={at={(ticklabel cs:0.5)},anchor=north},
% 	every axis y label/.style={at={(ticklabel cs:0.5)},rotate=90,anchor=south},
	every axis/.append style={font=\scriptsize},
	every axis plot/.append style={thick,mark size=1.2,tension=0.18},
	legend cell align=left, legend style={fill opacity=0.8}
}

\pgfplotsset{
	dash/.style={mark=o,dashed,opacity=0.7},
	dott/.style={mark=o,dotted,opacity=0.7},
	notick/.style={xtick=\empty,ytick=\empty,ztick=\empty},
	notic/.style={xticklabels={,,},yticklabels={,,},zticklabels={,,}},
	noxtic/.style={xticklabels={,,}},
	noytic/.style={yticklabels={,,}},
	noztic/.style={zticklabels={,,}},
	nolim/.style={enlargelimits=false},
	noxlim/.style={enlarge x limits=false},
	noylim/.style={enlarge y limits=false},
	nozlim/.style={enlarge z limits=false},
	lim/.style={enlargelimits=true},
	xlim/.style={enlarge x limits=true},
	ylim/.style={enlarge y limits=true},
	zlim/.style={enlarge z limits=true},
	ulim/.style={enlargelimits=upper},
	uxlim/.style={enlarge x limits=upper},
	uylim/.style={enlarge y limits=upper},
	uzlim/.style={enlarge z limits=upper},
% 	stealth/.style={grid=none,hide axis=true}, % alignment breaks
	stealth/.style={notick,axis line style={opacity=0}},
	plain/.style={every axis plot/.append style={},nolim,grid=none},
	comb/.style={every axis plot/.append style={ycomb,mark=*},noxlim,uylim,grid=none},
	cent/.style={axis lines=center},
	graf/.style={axis x line=bottom, axis y line=left},
	scat/.style={scatter,only marks,point meta=explicit},
	xy/.style={
		every axis x label/.style={at={(ticklabel* cs:1)},anchor=west},
		every axis y label/.style={at={(ticklabel* cs:1)},anchor=south},
	},
	xyz/.style={
		every axis x label/.style={at={(ticklabel* cs:1)},anchor=west},
		every axis y label/.style={at={(ticklabel* cs:1)},anchor=west},
		every axis z label/.style={at={(ticklabel* cs:1)},anchor=south},
	},
	z-sort/.style={z buffer=sort,unbounded coords=jump},
}

\newcommand{\igiga}[1]{\thisrowno{#1}/1000000000}
\newcommand{\imega}[1]{\thisrowno{#1}/1000000}
\newcommand{\ikilo}[1]{\thisrowno{#1}/1000}
\newcommand{\iperc}[2]{\thisrowno{#1}/#2}
\newcommand{\imap}[1]{\thisrow{#1}*100}
\newcommand{\giga}[1]{\thisrow{#1}/1000000000}
\newcommand{\mega}[1]{\thisrow{#1}/1000000}
\newcommand{\kilo}[1]{\thisrow{#1}/1000}
\newcommand{\perc}[2]{\thisrow{#1}/#2}
\newcommand{\map}[1]{\thisrow{#1}*100}

%------------------------------------------------------------------------------
% https://tex.stackexchange.com/a/355579/38641
% to use e.g. as "only=<4>{/pgf/bar width=2.8}" in axis options
\tikzset{only/.code args={<#1>#2}{\only<#1>{\pgfkeysalso{#2}}}}

%------------------------------------------------------------------------------
% python plots and plain axes

\newcommand{\python}[1]{python -c "%
import math, sys; import numpy as np; import scipy.linalg as la;%
#1 np.savetxt(sys.stdout, data)%
"}
\newcommand<>{\pyplot}[3][]%
{\only#4{\addplot[#1] shell[prefix=fig/data/,id=#2,] {\python{#3}};}}
\newcommand<>{\pyplott}[3][]%
{\only#4{\addplot3[z-sort,#1] shell[prefix=fig/data/,id=#2,] {\python{#3}};}}
\newcommand<>{\pyload}[3][]%
{\only#4{\addplot[#1] table[x index=0,y index=#2] {fig/data/#3.out};}}
\newcommand<>{\pyloadp}[3][]%
{\only#4{\addplot+[#1] table[x index=0,y index=#2] {fig/data/#3.out};}}
\newcommand<>{\pyloadt}[2][]%
{\only#3{\addplot3[z-sort,#1] table {fig/data/#2.out};}}
\newcommand{\pysave}[2]{
	\begin{tikzpicture}[overlay,opacity=0]
	\begin{axis} \pyplot{#1}{#2} \end{axis}
	\end{tikzpicture}
}
\newenvironment<>{axes}[3][plain]{
	\begin{onlyenv}#4
	\begin{tikzpicture}
	\begin{axis}[width=#2\textwidth,height=#3\textwidth,#1]
}{
	\end{axis}
	\end{tikzpicture}
	\end{onlyenv}
}
\newenvironment<>{xaxes}[3][plain]{
	\begin{onlyenv}#4
	\begin{tikzpicture}
	\begin{semilogxaxis}[width=#2\textwidth,height=#3\textwidth,#1]
}{
	\end{semilogxaxis}
	\end{tikzpicture}
	\end{onlyenv}
}
\newenvironment<>{xyaxes}[3][plain]{
	\begin{onlyenv}#4
	\begin{tikzpicture}
	\begin{loglogaxis}[width=#2\textwidth,height=#3\textwidth,#1]
}{
	\end{loglogaxis}
	\end{tikzpicture}
	\end{onlyenv}
}

%------------------------------------------------------------------------------
% python external plots with matplotlib & pgf

% convert unit of measure, e.g. \unit{in}{.8\textwidth}
\makeatletter
\def\unit#1#2{\strip@pt\dimexpr #2*65536/\number\dimexpr 1#1}
\makeatother

\newcommand{\pygf}[3]{python -c "%
import math, sys; import numpy as np; import scipy.linalg as la; %
import matplotlib as mpl; mpl.use('pgf'); import matplotlib.pyplot as plt; %
mpl.rcParams.update({'font.family':'serif','font.size':8}); %
fig = plt.figure(figsize=#2); #3 fig.savefig('#1', dpi=500); %
"}

\newcommand<>{\pygfplot}[4]{
	\immediate\write18{\pygf{fig/pgf/#1.pgf}{(\unit{in}{#2},\unit{in}{#3})}{#4}}
	\only#5{\input{fig/pgf/#1.pgf}}
}

%--------------------------------------------------------------------
% 2d drawing

% 2d coordinates
\def\bx(#1,#2){#1}
\def\by(#1,#2){#2}
\def\dx(#1,#2){#1,0}
\def\dy(#1,#2){0,#2}

% node coordinate system
\newcommand{\ncs}[2]{%
($(#1.south west)!\bx(#2)!(#1.south east)!\by(#2)!($(#1.north west)!\bx(#2)!(#1.north east)$)$)%
}

% rectangle in node coordinate system
\newcommand<>{\nrect}[4][]{\path#5[#1] \ncs{#2}{#3} rectangle \ncs{#2}{#4};}

% draw centered rectangle by node
\newcommand{\rectn}[4]{%
	node[draw,rectc,minimum width=#3cm,minimum height=#4cm,#1](#2){}%
}

% draw image by node
\newcommand{\rectim}[2]{%
	node[rect] {\graph[width={\bx(#1)}cm,height={\by(#1)}cm]{#2}}%
}

% draw image by node, with label
\newcommand{\rectiml}[3]{%
	node[rect](#1) {\graph[width={\bx(#2)}cm,height={\by(#2)}cm]{#3}}%
}

%------------------------------------------------------------------------------
% 3d drawing

\pgfkeys{/tikz/.cd, aspect/.store in=\aspect, aspect=3}
\pgfkeys{/tikz/.cd, depth/.store in=\depth, depth=.15}
\pgfkeys{/tikz/.cd, stepx/.store in=\step, stepx=1}

\tikzstyle{geom} = [line join=bevel,aspect=3,depth=.15,z={(\depth*\aspect,\depth)}]
\tikzstyle{wire} = [geom,draw,thick]

% 3d coordinates
\def\cx#1,#2,#3{#1}
\def\cy#1,#2,#3{#2}
\def\cz#1,#2,#3{#3}
\def\ex#1,#2,#3{#1,0,0}
\def\ey#1,#2,#3{0,#2,0}
\def\ez#1,#2,#3{0,0,#3}

% lines along x, y, or z
\newcommand{\zline}[3][]{%
\path[geom,#1] #2 -- +(\cx#3,\cy#3);
}
\newcommand{\yline}[3][]{%
\path[geom,#1,shift={#2},xslant=\aspect]
	(0,0) -- +(\cx#3,\depth*\cz#3);
}
\newcommand{\xline}[3][]{%
\path[geom,#1,shift={#2},yslant=1/\aspect]
	(0,0) -- +(\aspect*\depth*\cz#3,\cy#3);
}

% rectangles / grids along x, y, or z
\newcommand{\zrect}[3][]{%
\path[geom,#1] #2 rectangle +(\cx#3,\cy#3);
}
\newcommand{\yrect}[3][]{%
\path[geom,#1,shift={#2},xslant=\aspect]
	(0,0) rectangle +(\cx#3,\depth*\cz#3);
}
\newcommand{\xrect}[3][]{%
\path[geom,#1,shift={#2},yslant=1/\aspect]
	(0,0) rectangle +(\aspect*\depth*\cz#3,\cy#3);
}
\newcommand{\xgrid}[3][]{%
\path[geom,#1,shift={#2},yslant=1/\aspect,xstep=\aspect*\depth*\step]
	(0,0) grid +(\aspect*\depth*\cz#3,\cy#3);
}

% parallepiped
\newcommand{\para}[3][]{%
\zrect[#1]{(#2)}{#3}               % front
\yrect[#1]{($(#2)+(\ey#3)$)}{#3}   % top
\xrect[#1]{($(#2)+(\ex#3)$)}{#3}   % right
}

\newcommand{\xrectim}[4][]{%
\path[geom,#1,shift={#2},yslant=1/\aspect]
	let \n0={\aspect*\depth*\cz#3} in
		(0,0) node[rect] {\graph[width={\n0}cm,height={\cy#3}cm]{#4}};
}
\newcommand{\paraim}[4][]{%
\zrect[#1]{(#2)}{#3}                     % front
\yrect[#1]{($(#2)+(\ey#3)$)}{#3}         % top
\xrectim[#1]{($(#2)+(\ex#3)$)}{#3}{#4}   % right, image
\xrect[#1]{($(#2)+(\ex#3)$)}{#3}         % right
}

%------------------------------------------------------------------------------
% externalize

% \usepgfplotslibrary{external}
% % \tikzexternalize
% % \newcommand{\extfig}[2]{\tikzsetnextfilename{fig/extern/#1}{#2}}
% \tikzexternalize[prefix=fig/extern/]
% \newcommand{\extfig}[2]{\tikzsetnextfilename{#1}{#2}}
% \newcommand{\extdata}[1]{\input{#1}}


==> figs/low-pass/tex/slides.tex <==
\usetheme{default}
\definecolor{orng}{rgb}{1,.35,0}
\usecolortheme[named=orng]{structure}
\setbeamercolor{alerted text}{fg=orng}
\usefonttheme{structurebold}
\usefonttheme[onlymath]{serif}
\setbeamercovered{transparent}
\setbeamertemplate{frametitle}[default][center]
\setbeamertemplate{itemize items}[circle]
\setbeamersize{text margin left=10pt}
\setbeamersize{text margin right=10pt}

%--------------------------------------------------------------------
% FIGURES: CHOOSE ONE OPTION
%
% plots:     build standalone pdfs for figures, then use them
% plots-ext: use existing pds for figures
%
\input{tex/plots}
%  \input{tex/plots-ext}
%--------------------------------------------------------------------

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{tabularx}
\usepackage{array}
\usepackage{xspace}
\usepackage{multirow}
\usepackage{array}
\usepackage{setspace}
\usepackage{bbm}
\usepackage{varwidth}
\usepackage{multimedia}
\usepackage[]{animate}

\usepackage{enumitem}
\setlist[itemize]{label=\usebeamerfont*{itemize item}%
	\usebeamercolor[fg]{itemize item}%
	\usebeamertemplate{itemize item}%
}
\setlist[enumerate]{label=\protect\usebeamerfont*{enumerate item}%
	\protect\usebeamercolor[fg]{enumerate item}%
	\insertenumlabel%
}

%--------------------------------------------------------------------

\input{tex/abbrev}    % standard abbreviations
\input{tex/beam}      % macros for beamer


==> tex/ext-plots.tex <==
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage{pgf,tikz}

\usepackage{tikzextern}
%\usepackage{pgffor}
\newcommand{\extfig}[2]{\tikzsetnextfilename{figs/extern/#1}{#2}}
\newcommand{\extdata}[1]{}


==> tex/fig_intro.tex <==
%--------------------------------------------------------------------
\tikzset{
	axis/.style={gray,thin},
	arrow/.style={
		decoration={markings,mark=at position 1 with {\arrow[scale=.8]{>}}},
		postaction={decorate},
		shorten >=2pt,
	},
	dot/.style={draw,fill,circle,inner sep=.7pt},
	vertex/.style={draw=blue,fill=white,circle,inner sep=1pt},
	undir/.style={blue,thick},
	dir/.style={blue,thick,arrow},
}
%--------------------------------------------------------------------
\newcommand{\makeaxis}[1]{%
	% axes
	\draw[axis,->] (-1,0) -- (9,0) node[below] {$\scriptstyle i$};
	\draw[axis,->] (0,-1) -- (0,3) node[left]  {$\scriptstyle {#1}_i$};

	% x ticks
	\foreach \n in {1,2,...,8}
		\draw[axis] (\n,-.1) -- ++(0,.2);

	% y ticks
	\foreach \n in {1,2}
		\draw[axis] (-.1,\n) -- ++(.2,0);
}
%--------------------------------------------------------------------
\newcommand{\zgraph}{%
	% graph
	\node[left,blue] at (0,-.6) {$\scriptstyle G$};
	\foreach \n in {0,1,...,8}
		\node[vertex] (v\n) at (\n,-.6) {};
	\foreach \f/\t in {0/1,1/2,2/3,3/4,4/5,5/6,6/7,7/8}
		\draw[dir] (v\f) -- (v\t);
}
%--------------------------------------------------------------------
\newcommand{\ggraph}{%
	% graph
	\node[left,blue] at (0,-.6) {$\scriptstyle G$};
	\foreach \n in {0,1,...,4,6,7,8}
		\node[vertex] (v\n) at (\n,-.6) {};
	\foreach \f/\t in {0/1,1/2,2/3,3/4,6/7,7/8}
		\draw[undir] (v\f) -- (v\t);
}
%--------------------------------------------------------------------
\newcommand{\sigfig}[2]{%
	\hspace{-0pt}
	\extfig{#1}{
	\begin{tikzpicture}[>=latex',thick,scale=.35]
		{#2}
	\end{tikzpicture}
	} % extfig
	\hspace{-0pt}
}
%--------------------------------------------------------------------
\begin{figure}
{\setlength{\tabcolsep}{0pt}
\begin{tabular}{cc}
%--------------------------------------------------------------------
\sigfig{zin}{
	\makeaxis{y}
	\zgraph
	% signal
	\draw[thick,green] (2,0) -- ++(0,2) node[dot,red] {};
	\foreach \n in {0,1,3,4,...,8}
		\node[dot] at (\n,0) {};
}
%--------------------------------------------------------------------
&
%--------------------------------------------------------------------
\sigfig{zout}{
	\makeaxis{x}
	\zgraph
	% signal
	\foreach \n in {0,1}
		\node[dot] at (\n,0) {};
	\foreach \n [evaluate=\n as \v using 2*.9^(\n-2)] in {2,3,...,8}
		\draw[thick] (\n,0) -- ++(0,\v) node[dot] {};
}
%--------------------------------------------------------------------
\\ (a) & (b) \\
%--------------------------------------------------------------------
\sigfig{gin}{
	\makeaxis{y}
	% signal
	\ggraph
	\draw[thick,red] (2,0) -- ++(0,2) node[dot,red] {};
	\foreach \n in {0,1,3,4,6,7,8}
		\node[dot] at (\n,0) {};
}
%--------------------------------------------------------------------
&
%--------------------------------------------------------------------
\sigfig{gout}{
	\makeaxis{x}
	\ggraph
	% signal
	\foreach \n [evaluate=\n as \v using 2*.9^abs(\n-2)] in {0,1,...,4}
		\draw[thick] (\n,0) -- ++(0,\v) node[dot] {};
	\foreach \n in {6,7,8}
		\node[dot] at (\n,0) {};
}
%--------------------------------------------------------------------
\\ (c) & (d)
\end{tabular}
} % tabcolsep
\caption{(a) Input signal $y_i \defn 2\delta_{i-2}, \ i \in \zahl$. (b) Output signal $x_i \defn \beta \sum_{t=0}^\infty \alpha^t y_{i-t}$ with $\alpha \in [0,1)$ and $\beta \defn 1 - \alpha$, corresponding to a low-pass filter determined by the equation $x_i = \alpha x_{i-1} + (1-\alpha) y_i$. Its (infinite) impulse response $h_t = \beta \alpha^t u_t$ and transfer function $H_\alpha(z) \defn \beta \sum_{t=0}^\infty (az^{-1})^t = \beta / (1 - \alpha z^{-1})$.
%$\delta, u$ are the discrete-time unit impulse and step functions respectively.
This assumes a directed graph $G$ with vertices $V = \zahl$ and edges $E = \{(i,i+1): i \in \zahl\}$, shown in blue. (c), (d) use an
%Using an arbitrary finite, weighted,
undirected graph $G$ instead. Information ``flows'' in all directions, controlled by edge weights.
%In retrieval, the sample in red represents the query, and the output $x$ is its similarity to all samples.
We perform image retrieval efficiently as filtering in the frequency domain.
}
\label{fig:idea}
\end{figure}


==> tex/no-plots.tex <==
\newcommand{\extfig}[2]{!}
\newcommand{\extdata}[1]{}

